AML-SVM: Adaptive Multilevel Learning with Support Vector Machines

The support vector machines (SVM) is one of the most widely used and practical optimization based classification models in machine learning because of its interpretability and flexibility to produce high quality results. However, the big data imposes a certain difficulty to the most sophisticated but relatively slow versions of SVM, namely, the nonlinear SVM. The complexity of nonlinear SVM solvers and the number of elements in the kernel matrix quadratically increases with the number of samples in training data. Therefore, both runtime and memory requirements are negatively affected. Moreover, the parameter fitting has extra kernel parameters to tune, which exacerbate the runtime even further. This paper proposes an adaptive multilevel learning framework for the nonlinear SVM, which addresses these challenges, improves the classification quality across the refinement process, and leverages multi-threaded parallel processing for better performance. The integration of parameter fitting in the hierarchical learning framework and adaptive process to stop unnecessary computation significantly reduce the running time while increase the overall performance. The experimental results demonstrate reduced variance on prediction over validation and test data across levels in the hierarchy, and significant speedup compared to state-of-the-art nonlinear SVM libraries without a decrease in the classification quality. The code is accessible at https://github.com/esadr/amlsvm.

==> algorithm_commands.tex <==
% https://tex.stackexchange.com/a/216139/82506
\newcommand{\var}[1]{\text{\texttt{#1}}}
\newcommand{\func}[1]{\text{\textsl{#1}}}

\makeatletter
\newcounter{phase}[algorithm]
\newlength{\phaserulewidth}
\newcommand{\setphaserulewidth}{\setlength{\phaserulewidth}}
\newcommand{\phase}[1]{%
  \vspace{-1.25ex}
  % Top phase rule
  \Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}
%   \Statex\strut\refstepcounter{phase}\textit{Phase~\thephase~--~#1}% Phase text
    \Statex\strut\refstepcounter{phase}\textit{#1}% Phase text
  % Bottom phase rule
  \vspace{-1.25ex}\Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}}
\makeatother

\setphaserulewidth{.5pt}

==> conf_template_content.tex <==

% \section{Problem Specification.}In this paper, we consider the solution of the $N \times
% N$ linear
% system
% \begin{equation} \label{e1.1}
% A x = b
% \end{equation}
% where $A$ is large, sparse, symmetric, and positive definite.  We consider
% the direct solution of (\ref{e1.1}) by means of general sparse Gaussian
% elimination.  In such a procedure, we find a permutation matrix $P$, and
% compute the decomposition
% \[
% P A P^{t} = L D L^{t}
% \]
% where $L$ is unit lower triangular and $D$ is diagonal.


% \section{Design Considerations.}Several good ordering algorithms (nested dissection and
% minimum degree)
% are available for computing $P$  \cite{GEORGELIU}, \cite{ROSE72}.
% Since our interest here does not
% focus directly on the ordering, we assume for convenience that $P=I$,
% or that $A$ has been preordered to reflect an appropriate choice of $P$.

% Our purpose here is to examine the nonnumerical complexity of the
% sparse elimination algorithm given in  \cite{BANKSMITH}.
% As was shown there, a general sparse elimination scheme based on the
% bordering algorithm requires less storage for pointers and
% row/column indices than more traditional implementations of general
% sparse elimination.  This is accomplished by exploiting the m-tree,
% a particular spanning tree for the graph of the filled-in matrix.

% \begin{theorem} The method  was extended to three
% dimensions. For the standard multigrid
% coarsening
% (in which, for a given grid, the next coarser grid has $1/8$
% as many points), anisotropic problems require plane
% relaxation to
% obtain a good smoothing factor.\end{theorem}

% Our purpose here is to examine the nonnumerical complexity of the
% sparse elimination algorithm given in  \cite{BANKSMITH}.
% As was shown there, a general sparse elimination scheme based on the
% bordering algorithm requires less storage for pointers and
% row/column indices than more traditional implementations of general
% sparse elimination.  This is accomplished by exploiting the m-tree,
% a particular spanning tree for the graph of the filled-in matrix.
% Several good ordering algorithms (nested dissection and minimum degree)
% are available for computing $P$  \cite{GEORGELIU}, \cite{ROSE72}.
% Since our interest here does not
% focus directly on the ordering, we assume for convenience that $P=I$,
% or that $A$ has been preordered to reflect an appropriate choice of $P$.

% \begin{proof} In this paper we consider two methods. The first method
% is
% basically the method considered with two differences:
% first, we perform plane relaxation by a two-dimensional
% multigrid method, and second, we use a slightly different
% choice of
% interpolation operator, which improves performance
% for nearly singular problems. In the second method coarsening
% is done by successively coarsening in each of the three
% independent variables and then ignoring the intermediate
% grids; this artifice simplifies coding considerably.
% \end{proof}

% Our purpose here is to examine the nonnumerical complexity of the
% sparse elimination algorithm given in  \cite{BANKSMITH}.
% As was shown there, a general sparse elimination scheme based on the
% bordering algorithm requires less storage for pointers and
% row/column indices than more traditional implementations of general
% sparse elimination.  This is accomplished by exploiting the m-tree,
% a particular spanning tree for the graph of the filled-in matrix.

% \begin{Definition}{\rm We describe the two methods in \S 1.2. In \S\ 1.3. we
% discuss
% some remaining details.}
% \end{Definition}

% Our purpose here is to examine the nonnumerical complexity of the
% sparse elimination algorithm given in  \cite{BANKSMITH}.
% As was shown there, a general sparse elimination scheme based on the
% bordering algorithm requires less storage for pointers and
% row/column indices than more traditional implementations of general
% sparse elimination.  This is accomplished by exploiting the m-tree,
% a particular spanning tree for the graph of the filled-in matrix.
% Several good ordering algorithms (nested dissection and minimum degree)
% are available for computing $P$  \cite{GEORGELIU}, \cite{ROSE72}.
% Since our interest here does not
% focus directly on the ordering, we assume for convenience that $P=I$,
% or that $A$ has been preordered to reflect an appropriate choice of $P$.

% Our purpose here is to examine the nonnumerical complexity of the
% sparse elimination algorithm given in  \cite{BANKSMITH}.
% As was shown there, a general sparse elimination scheme based on the
% bordering algorithm requires less storage for pointers and
% row/column indices than more traditional implementations of general
% sparse elimination.

% \begin{lemma} We discuss first the choice for $I_{k-1}^k$
% which is a generalization. We assume that $G^{k-1}$ is
% obtained
% from $G^k$
% by standard coarsening; that is, if $G^k$ is a tensor product
% grid $G_{x}^k \times G_{y}^k \times G_{z}^k$,
% $G^{k-1}=G_{x}^{k-1} \times G_{y}^{k-1} \times G_{z}^{k-1}$,
% where $G_{x}^{k-1}$ is obtained by deleting every other grid
% point of $G_x^k$ and similarly for $G_{y}^k$ and $G_{z}^k$.
% \end{lemma}

% To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6]. In \S 1.3., we analyze the complexity of the old and new
% approaches to the intersection problem for the special case of
% an $n \times n$ grid ordered by nested dissection. The special
% structure of this problem allows us to make exact estimates of
% the complexity. To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6].

% In \S 1.2, we review the bordering algorithm, and introduce
% the sorting and intersection problems that arise in the
% sparse formulation of the algorithm.
% In \S 1.3., we analyze the complexity of the old and new
% approaches to the intersection problem for the special case of
% an $n \times n$ grid ordered by nested dissection. The special
% structure of this problem allows us to make exact estimates of
% the complexity. To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6].


% For the old approach, we show that the
% complexity of the intersection problem is $O(n^{3})$, the same
% as the complexity of the numerical computations.  For the
% new approach, the complexity of the second part is reduced to
% $O(n^{2} (\log n)^{2})$.

% To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6]. In \S 1.3., we analyze the complexity of the old and new
% approaches to the intersection problem for the special case of
% an $n \times n$ grid ordered by nested dissection. The special
% structure of this problem allows us to make exact estimates of
% the complexity. To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6].
% This is accomplished by exploiting the m-tree,
% a particular spanning tree for the graph of the filled-in matrix.
% To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% \cite{EISENSTAT} - \cite{LIU2}, \cite{ROSE76},  \cite{SCHREIBER}.

% \subsection{Robustness.}We do not
% attempt to present an overview
% here, but rather attempt to focus on those results that
% are relevant to our particular algorithm.
% This section assumes prior knowledge of the role of graph theory
% in sparse Gaussian elimination; surveys of this role are
% available in \cite{ROSE72} and \cite{GEORGELIU}. More general
% discussions of elimination trees are given in
% \cite{LAW} - \cite{LIU2}, \cite{SCHREIBER}.
% Thus, at the $k$th stage, the bordering algorithm consists of
% solving the lower triangular system
% \begin{equation} \label{1.2}
%  L_{k-1}v = c
% \end{equation}
% and setting
% \begin{eqnarray}
% \ell &=& D^{-1}_{k-1}v , \\
% \delta &=& \alpha - \ell^{t} v .
% \end{eqnarray}

% \begin{figure}
% \vspace{14pc}
% \caption{This is a figure 1.1.}
% \end{figure}

% \section{Robustness.} We do not
% attempt to present an overview
% here, but rather attempt to focus on those results that
% are relevant to our particular algorithm.

% \subsection{Versatility.}The special
% structure of this problem allows us to make exact estimates of
% the complexity.  For the old approach, we show that the
% complexity of the intersection problem is $O(n^{3})$, the same
% as the complexity of the numerical computations
% \cite{GEORGELIU}, \cite{ROSEWHITTEN}.  For the
% new approach, the complexity of the second part is reduced to
% $O(n^{2} (\log n)^{2})$.

% To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6]. In \S 1.3., we analyze the complexity of the old and new
% approaches to the intersection problem for the special case of
% an $n \times n$ grid ordered by nested dissection. The special
% structure of this problem allows us to make exact estimates of
% the complexity. To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6].

% In \S 1.2, we review the bordering algorithm, and introduce
% the sorting and intersection problems that arise in the
% sparse formulation of the algorithm.
% In \S 1.3., we analyze the complexity of the old and new
% approaches to the intersection problem for the special case of
% an $n \times n$ grid ordered by nested dissection. The special
% structure of this problem allows us to make exact estimates of
% the complexity. To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6].


% For the old approach, we show that the
% complexity of the intersection problem is $O(n^{3})$, the same
% as the complexity of the numerical computations.  For the
% new approach, the complexity of the second part is reduced to
% $O(n^{2} (\log n)^{2})$.

% To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6]. In \S 1.3., we analyze the complexity of the old and new
% approaches to the intersection problem for the special case of
% an $n \times n$ grid ordered by nested dissection. The special
% structure of this problem allows us to make exact estimates of
% the complexity. To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% [4] - [10], [5], [6].
% This is accomplished by exploiting the m-tree,
% a particular spanning tree for the graph of the filled-in matrix.
% To our knowledge, the m-tree previously has not been applied in this
% fashion to the numerical factorization, but it has been used,
% directly or indirectly, in several optimal order algorithms for
% computing the fill-in during the symbolic factorization phase
% \cite{EISENSTAT} - \cite{LIU2}, \cite{ROSE76},  \cite{SCHREIBER}.



% \begin{thebibliography}{99}

% %\bibitem{GUIDE}
% %R.~E. Bank, {\em PLTMG  users' guide, edition 5.0}, tech. report,
% %  Department of Mathematics, University of California, San Diego, CA, 1988.

% %\bibitem{HBMG}
% %R.~E. Bank, T.~F. Dupont, and H.~Yserentant, {\em The hierarchical basis
% %  multigrid method}, Numer. Math., 52 (1988), pp.~427--458.

% \bibitem{BANKSMITH}
% R.~E. Bank and R.~K. Smith, {\em General sparse elimination requires no
%   permanent integer storage}, SIAM J. Sci. Stat. Comput., 8 (1987),
%   pp.~574--584.

% \bibitem{EISENSTAT}
% S.~C. Eisenstat, M.~C. Gursky, M.~Schultz, and A.~Sherman, {\em
%   Algorithms and data structures for sparse symmetric gaussian elimination},
%   SIAM J. Sci. Stat. Comput., 2 (1982), pp.~225--237.

% \bibitem{GEORGELIU}
% A.~George and J.~Liu, {\em Computer Solution of Large Sparse Positive
%   Definite Systems}, Prentice Hall, Englewood Cliffs, NJ, 1981.

% \bibitem{LAW}
% K.~H. Law and S.~J. Fenves, {\em A node addition model for symbolic
%   factorization}, ACM TOMS, 12 (1986), pp.~37--50.

% \bibitem{LIU}
% J.~W.~H. Liu, {\em A compact row storage scheme for cholesky factors
%   using elimination trees}, ACM TOMS, 12 (1986), pp.~127--148.

% \bibitem{LIU2}
% \sameauthor , {\em The role of
%   elimination trees in sparse factorization}, Tech. Report CS-87-12,Department
%   of Computer Science, York University, Ontario, Canada, 1987.

% \bibitem{ROSE72}
% D.~J. Rose, {\em A graph theoretic study of the numeric solution of
%   sparse positive definite systems}, in Graph Theory and Computing, Academic  Press, New
% York, 1972.

% \bibitem{ROSE76}
% D.~J. Rose, R.~E. Tarjan, and G.~S. Lueker, {\em Algorithmic aspects of
%   vertex elimination on graphs}, SIAM J. Comput., 5 (1976), pp.~226--283.

% \bibitem{ROSEWHITTEN}
% D.~J. Rose and G.~F. Whitten, {\em A recursive analysis of disection
%   strategies}, in Sparse Matrix Computations, Academic Press, New York, 1976.

% \bibitem{SCHREIBER}
% R.~Schrieber, {\em A new implementation of sparse gaussian elimination},
%   ACM TOMS, 8 (1982), pp.~256--276.

% \end{thebibliography}


==> custom_commands.tex <==
\RequirePackage{fix-cm}
% \smartqed  % flush right qed marks, e.g. at end of proof
\usepackage{multirow}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{algpseudocode}
% \usepackage{ltexpprt}
\usepackage[utf8]{inputenc}
\usepackage{array}
\usepackage{graphicx,color,enumerate}
\usepackage{hyperref}
\usepackage{graphicx}
% \usepackage{wrapfig,lipsum,booktabs,caption}
\usepackage{varwidth}% http://ctan.org/pkg/varwidth
\usepackage[ruled]{algorithm} %commented 112319_1625
\usepackage{epstopdf}
\usepackage{capt-of}% or \usepackage{caption}
\usepackage{longtable}
\usepackage{printlen} 
%-------------------- preface ------------------------------

%\usepackage{amsmath,amssymb,ulsy,multicol}

\newcommand{\OO}{\mathcal{O}}

\newcommand{\JJ}{\mathcal{J}}
\newcommand{\JJFP}{\mathcal{J}^+_{all}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\CC}{{\textbf C}} 
\newcommand{\DD}{{\textbf D}} % data points
\newcommand{\GNode}{{\textbf V}} % vertex in graph


\newcommand{\coarsen}{\textsf{coarsen}$-\bullet$}
\newcommand{\uncoarsen}{\textsf{uncoarsen}$-\bullet$}
\newcommand{\refine}{\textsf{refine}$-\bullet$}

\newcommand{\mlsvm}{\textsf{mlsvm}}
\newcommand{\sv}{\textsf{sv}}
\newcommand{\params}{\textsf{$\pi$}}

\newcommand{\VV}{\mathcal{V}}
\newcommand{\FP}{\mathcal{F}_p}
\newcommand{\FN}{\mathcal{F}_n}

\newenvironment{proofsk}[1][\proofname]{\proof[#1]}{\endproof}

%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\textbfseries #1}]}{\end{trivlist}}
\pagestyle{empty}

%\newtheorem*{myclaim}{Claim}
%\newtheorem*{myex}{Example}

\usepackage{graphicx}
\usepackage{calc}
\newlength{\depthofsumsign}
\setlength{\depthofsumsign}{\depthof{$\sum$}}
\newlength{\totalheightofsumsign}
\newlength{\heightanddepthofargument}

\newcommand{\nsum}[1][1.4]{% only for \displaystyle
    \mathop{%
        \raisebox
            {-#1\depthofsumsign+1\depthofsumsign}
            {\scalebox
                {#1}
                {$\displaystyle\sum$}%
            }
    }
}
\newcommand{\resum}[1]{%
    \def\s{#1}
    \mathop{
        \mathpalette\resumaux{#1}
    }
}

\newcommand{\resumaux}[2]{% internally
    \sbox0{$#1#2$}
    \sbox1{$#1\sum$}
    \setlength{\heightanddepthofargument}{\wd0+\dp0}
    \setlength{\totalheightofsumsign}{\wd1+\dp1}
    \def\quot{\DivideLengths{\heightanddepthofargument}{\totalheightofsumsign}}
    \nsum[\quot]%
}

% http://tex.stackexchange.com/a/6424/16595
\makeatletter
\newcommand*{\DivideLengths}[2]{%
  \strip@pt\dimexpr\number\numexpr\number\dimexpr#1\relax*65536/\number\dimexpr#2\relax\relax sp\relax
}
\makeatother

%\newtheorem*{theorem*}{Theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem*{lem*}{Lemma}

\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

%===============================================
\newcommand{\mb}[1]{\mbox{\boldmath $#1$}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\blambda}{\mbox{\boldmath$\lambda$}}
\newcommand{\bxi}{\mbox{\boldmath$\xi$}}
\newcommand{\bvi}{\mbox{\boldmath$\upsilon$}}
\newcommand{\bA}{\mb{A}}
\newcommand{\bB}{B}
\newcommand{\bC}{C}
\newcommand{\bD}{D}
\newcommand{\bb}{\mb{b}}
\newcommand{\bc}{c}
\newcommand{\vi}{\upsilon}
\newcommand{\bw}{\mb{w}}
\newcommand{\bx}{\mb{x}}
\newcommand{\vx}{\mb{v}}
\newcommand{\be}{\mb{e}}
\newcommand{\by}{\mb{y}}
\newcommand{\bp}{\mb{p}}
\newcommand{\bu}{\mb{u}}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\half}{\hbox{$\frac{1}{2}$}}
\newcommand{\hsp}{\hspace{0.2in}}
\newcommand{\onurcomment}[1]{{\color{blue} \{\bf{\emph{#1}}\}}}


==> large_results.tex <==
\def \subplotW{0.48\linewidth}
\def \subplotH{12pc}
\def \subplotBelowHeader{\amlHeaderUp}
\def \subplotHeaderH{1.5pc}
\def \subtextW{0.02\linewidth}
\def \subimgsize{\textwidth}
% \def \subplotLiftUp{-2.6pc}
\def \subplotLiftUp{\amlLiftUp}

\onecolumn
\begin{table*}[htb]
    \centering
    \vspace{\subplotLiftUp}
    \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
    \hline
        &\begin{minipage}[c][\subplotHeaderH]{\subtextW} \centering
            Name
        \end{minipage}  
        \begin{minipage}[c][\subplotHeaderH]{\subplotW} \centering
            Average
        \end{minipage} 
        \begin{minipage}[c][\subplotHeaderH]{\subplotW} \centering
            Sample
        \end{minipage}  \\ \hline
        \vspace{\subplotBelowHeader}
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Advertisement}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_3_levels_advertisement} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_393463_advertisement} 
        \end{minipage}  %\\ \hline
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Buzz}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_7_levels_buzz} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_883788_buzz} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Clean}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_5_levels_clean} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_827147_clean} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Cod-RNA}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_7_levels_cod} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_883788_cod} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------    
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Forest}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_9_levels_forest} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_883788_forest} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------
    \caption{Comparing the prediction quality across levels, part 1}
    \label{tab:aml_plots_part1}
\end{table*}    
    
    
\onecolumn
\begin{table*}[htb]
    \centering
    \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
    \hline
        &\begin{minipage}[c][\subplotHeaderH]{\subtextW} \centering
            Name
        \end{minipage}  
        \begin{minipage}[c][\subplotHeaderH]{\subplotW} \centering
            Average
        \end{minipage} 
        \begin{minipage}[c][\subplotHeaderH]{\subplotW} \centering
            Sample
        \end{minipage}  \\ \hline
        \vspace{\subplotBelowHeader}
    \end{tabular*}
%-----------------------------------------------------------------------------    
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Letter}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_6_levels_letter} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_495302_letter} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Ringnorm}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_4_levels_ringnorm} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_3390_ringnorm} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------    
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{Twonorm}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_4_levels_twonorm} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_495302_twonorm} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{HIGGS}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_14_levels_higgs} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_424321_higgs} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------
\vspace{\subplotLiftUp}
\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
        &\begin{minipage}[c][\subplotH]{\subtextW} \centering
            \rotatebox[origin=c]{90}{SUSY}
        \end{minipage}  
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/agg_13_levels_susy} 
        \end{minipage} 
        \begin{minipage}[c][\subplotH]{\subplotW} \centering
            \includegraphics[width=\subimgsize]{plots/indv_cmid_729771_susy} 
        \end{minipage}  \\ %\hline
    \end{tabular*}
%-----------------------------------------------------------------------------    
    \caption{Comparing the prediction quality across levels, part 2}
    \label{tab:aml_plots_part2}
\end{table*}    

\twocolumn

==> unused_results.tex <==
\begin{table*}[!ht]
%   \footnotesize
  \setlength{\tabcolsep}{4pt}
  \caption{Performance measures for LIBSVM, DC-SVM, ML-SVM and AML-SVM on benchmark data sets.}
  \label{tab:aml_mlsvm_journal_paper_medium_data_time_performance_measures}
  %\vspace{-.5cm}
  \begin{center}
    \scalebox{.75}{
    \begin{tabular}{lcccc|cccc|cccc|cccc}
      \hline
       & \multicolumn{4}{c|}{LIBSVM} & \multicolumn{4}{c|}{DC-SVM} & \multicolumn{4}{c|}{ML-SVM} 
       & \multicolumn{4}{c}{AML-SVM} \\ \cline{2-17}
      Datasets      & ACC & SN & SP & G-mean            & ACC & SN & SP & G-mean        & ACC & SN & SP & G-mean          & ACC & SN & SP & G-mean\\ \hline
	Advertisement   & 0.92 & 0.99 & 0.45 & 0.67         & 0.95 & 0.83 & 0.97 & 0.90        & 0.95 & 0.85 & 0.96 & \bf{0.91}  & 0.93 & 0.86 & 0.94 & 0.90   \\
	Buzz            & 0.96 & 0.99 & 0.81 & 0.89         & 0.96 & 0.88 & 0.97 & 0.92        & 0.94 & 0.95 & 0.94 & \bf{0.95}  & 0.94 & 0.97 & 0.93 & \bf{0.95} \\
	Clean (Musk)    & 1.00 & 1.00 & 0.98 & \bf{0.99}    & 0.96 & 0.91 & 0.97 & 0.94        & 0.99 & 0.99 & 0.99 & \bf{0.99}  & 0.95 & 0.91 & 0.96 & 0.93   \\
	Cod-RNA         & 0.96 & 0.96 & 0.96 & \bf{0.96}    & 0.93 & 0.93 & 0.94 & 0.93        & 0.93 & 0.97 & 0.91 & 0.94       & 0.94 & 0.97 & 0.93 & 0.95   \\
	Forest          & 1.00 & 1.00 & 0.86 & 0.92         & 1.00 & 0.88 & 1.00 & \bf{0.94}   & 0.77 & 0.96 & 0.80 & 0.88       & 0.84 & 0.93 & 0.84 & 0.88   \\
	Letter          & 1.00 & 1.00 & 0.97 & 0.99         & 1.00 & 1.00 & 1.00 & \bf{1.00}   & 0.98 & 0.99 & 0.98 & 0.99       & 0.99 & 0.96 & 0.99 & 0.98   \\
	Ringnorm        & 0.98 & 0.99 & 0.98 & \bf{0.98}    & 0.95 & 0.92 & 0.98 & 0.95        & 0.98 & 0.98 & 0.98 & \bf{0.98}  & 0.97 & 0.98 & 0.96 & 0.97   \\
	Twonorm         & 0.98 & 0.98 & 0.99 & \bf{0.98}    & 0.97 & 0.98 & 0.96 & 0.97        & 0.98 & 0.98 & 0.97 & \bf{0.98}  & 0.97 & 0.98 & 0.96 & 0.97   \\ \hline
    \end{tabular}}
  \end{center}
  \normalsize
\end{table*}


\begin{table*}[!ht]
  \normalsize
  \caption{Computational time in seconds for LIBSVM, DC-SVM, ML-SVM and AML-SVM.} 
  \label{tab:aml_mlsvm_journal_paper_medium_data_time}
  \begin{center}
    \scalebox{1}{
      \begin{tabular}{lcccc}	\hline
	    Dataset         & LIBSVM     & DC-SVM   & ML-SVM     & AML-SVM  \\	\hline
	    Advertisement   & 231        & 610      &  213           & \bf{126}   \\
	    Buzz            & 26026      & 2524     &  \bf{31 }      & 269        \\
	    Clean (Musk)    & 82         & 95       &  94            & \bf{21}    \\
	    Cod-RNA         & 1857       & 420      &  \bf{13  }     & 75         \\
	    Forest          & 353210     & 19970    &  \bf{948}      & 2149       \\
	    Letter          & 139        & 38       &  30            & \bf{14}    \\
	    Ringnorm        & 26         & 38       &  \bf{2 }       & 3          \\
	    Twonorm         & 28         & 30       &  \bf{1 }       & \bf{1}     \\	\hline
      \end{tabular}}
  \end{center}
  \normalsize
\end{table*}





% \def \subplotW{0.44\linewidth}
% \def \subplotH{12pc}
% \def \subplotHeaderH{1pc}
% \def \subtextW{0.06\linewidth}
% \def \subimgsize{\textwidth}
% % \def \subplotLiftUp{-2.6pc}
% \def \subplotLiftUp{-2.5pc}

% \begin{table*}[htb]
%     \centering
%     % \vspace{\subplotLiftUp}
%     % \begin{tabularx}{\textwidth}
%     %     \centering{Average performance measures for refinement levels}
%     %     % \hline
%     % \end{tabularx}
% %-----------------------------------------------------------------------------
% % \vspace{\subplotLiftUp}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Advertisement}
%         \end{minipage}  
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_3_levels_advertisement} 
%         \end{minipage} 
%         % \vrule{}
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_7_levels_buzz} 
%         \end{minipage}  %\\ \hline
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Buzz}
%         \end{minipage}  
%     \end{tabular*}
% %-----------------------------------------------------------------------------
% % \vspace{-3pc}
% \vspace{\subplotLiftUp}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Clean}
%         \end{minipage}  
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_5_levels_clean} 
%         \end{minipage} 
%         % \vrule{}
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_7_levels_cod} 
%         \end{minipage}  %\\ \hline
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Cod}
%         \end{minipage}  
%     \end{tabular*}
% %-----------------------------------------------------------------------------
% \vspace{\subplotLiftUp}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Forest}
%         \end{minipage}  
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_9_levels_forest} 
%         \end{minipage} 
%         % \vrule{}
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_6_levels_letter.png} 
%         \end{minipage}  %\\ \hline
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Letter}
%         \end{minipage}  
%     \end{tabular*}
% %-----------------------------------------------------------------------------
% \vspace{\subplotLiftUp}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Ringnorm}
%         \end{minipage}  
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_4_levels_ringnorm.png} 
%         \end{minipage} 
%         % \vrule{}
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_4_levels_twonorm.png} 
%         \end{minipage}  %\\ \hline
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{Twonorm}
%         \end{minipage}  
%     \end{tabular*}
% %-----------------------------------------------------------------------------
%     \caption{Performance measure comparison between Normal (ML-SVM) and Adaptive (AML-SVM) methods across refinement's level for medium size datasets.}
%     \label{tab:aml_plots_agg_part1}
% \end{table*}    

% \begin{table*}[htb]
%     \centering

% \vspace{\subplotLiftUp}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{HIGGS - 10 levels}
%         \end{minipage}  
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_10_levels_higgs.png} 
%         \end{minipage}
        
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_11_levels_higgs.png} 
%         \end{minipage} 
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{HIGGS - 11 levels}
%         \end{minipage}  
%     \end{tabular*}
% %-----------------------------------------------------------------------------
% \vspace{\subplotLiftUp}
% \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{HIGGS - 14 levels}
%         \end{minipage}  
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_14_levels_higgs.png} 
%         \end{minipage} 
%         % \vrule{}
%         \begin{minipage}[c][\subplotH]{\subplotW} \centering
%             \includegraphics[width=\subimgsize]{plots/agg_13_levels_susy.png} 
%         \end{minipage}  %\\ \hline
%         \begin{minipage}[c][\subplotH]{\subtextW} \centering
%             \rotatebox[origin=c]{90}{SUSY - 13 levels}
%         \end{minipage}  
%     \end{tabular*}
% %-----------------------------------------------------------------------------

    
% %-----------------------------------------------------------------------------
%     \caption{Performance measure comparison between Normal (ML-SVM) and Adaptive (AML-SVM) methods across refinement's level for large scale datasets.}
%     \label{tab:aml_plots_agg_part1}
% \end{table*}    



% \begin{table*}[ht]
%     \centering
%     \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
%     \hline
%         &\begin{minipage}[c][\subplotHeaderH]{\subtextW} \centering
%             Name
%         \end{minipage}  
%         \begin{minipage}[c][\subplotHeaderH]{\subplotW} \centering
%             Average
%         \end{minipage} 
%         \begin{minipage}[c][\subplotHeaderH]{\subplotW} \centering
%             Sample
%         \end{minipage}   \\  \hline
%     \end{tabular*}
% %-----------------------------------------------------------------------------    
% % %-----------------------------------------------------------------------------
% % \vspace{\subplotLiftUp}
% % \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
% %         &\begin{minipage}[c][\subplotH]{\subtextW} \centering
% %             \rotatebox[origin=c]{90}{HIGGS}
% %         \end{minipage}  
% %         \begin{minipage}[c][\subplotH]{\subplotW} \centering
% %             \includegraphics[width=\subimgsize]{plots/agg_14_levels_higgs} 
% %         \end{minipage} 
% %         \begin{minipage}[c][\subplotH]{\subplotW} \centering
% %             \includegraphics[width=\subimgsize]{plots/indv_cmid_424321_higgs} 
% %         \end{minipage}  \\ %\hline
% %     \end{tabular*}
% % %-----------------------------------------------------------------------------
% % \vspace{\subplotLiftUp}
% % \begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} c}
% %         &\begin{minipage}[c][\subplotH]{\subtextW} \centering
% %             \rotatebox[origin=c]{90}{SUSY}
% %         \end{minipage}  
% %         \begin{minipage}[c][\subplotH]{\subplotW} \centering
% %             \includegraphics[width=\subimgsize]{plots/agg_13_levels_susy} 
% %         \end{minipage} 
% %         \begin{minipage}[c][\subplotH]{\subplotW} \centering
% %             \includegraphics[width=\subimgsize]{plots/indv_cmid_729771_susy} 
% %         \end{minipage}  \\ %\hline
% %     \end{tabular*}
% %-----------------------------------------------------------------------------    
%     \caption{Caption}
%     \label{tab:aml_plots_part3}
% \end{table*}

% \begin{minipage}[t]{0.43\textwidth}
% \includegraphics[width=\subimgsize]{plots/agg_4_levels_twonorm}
% \end{minipage}
% \begin{minipage}[t]{0.43\textwidth}
% \includegraphics[width=\subimgsize]{plots/agg_11_levels_susy}
% \end{minipage}


% forest agg 9 levels 
% higgs agg 14 levels 

% \begin{table*}[!ht]
%   \label{tab:aml_mlsvm_early_stop_time}
%  % \vspace{-.5cm}
%   \begin{center}
%     \scalebox{.9}{
%       \begin{tabular}{cccc}     \hline
%         Dataset    & Threshold (G-mean)  &ML-SVM Time & AML-SVM Time \\ \hline
%         Advertisement	 	&0.85	 &10.4	&15.0 	 \\
%         Buzz	 	&0.90	 &21.6	&22.2 	 \\
%         Clean (Musk)	 	&0.90	 &2.8	&3.5 	 \\
%         Cod-RNA	 	&0.90	 &2.6	&2.7 	 \\
%         Forest	 	&0.85	 &318.2	&253.2 	 \\
%         Letter	 	&0.95	 &1.6	&1.6 	 \\
%         Ringnorm	 	&0.95	 &2.7	&2.5 	 \\
%         Twonorm	 	&0.95	 &0.6	&0.6 	 \\
%         HIGGS	 	&0.60	 &408.2	&457.5 	 \\
%         SUSY	 	&0.70	 &223.9	&228.7 	 \\
%       \end{tabular}}
%   \end{center}
  
%   \caption{Average time (seconds) for early termination over all the configurations for each dataset with respect to the defined threshold.} 
% \end{table*}




	
% \begin{table*}[!ht]
%   \label{tab:aml_mlsvm_journal_paper_medium_data_time_performance_measures_dup}
%   %\vspace{-.5cm}
%   \begin{center}
%     \scalebox{.8}{
%     \begin{tabular}{lcccc|cccc}
%       \hline
%       & \multicolumn{4}{c|}{G-mean} & \multicolumn{4}{c}{Time} \\ \cline{2-9}
%     Datasets        & LIBSVM     & DC-SVM     & ML-SVM     & AML-SVM   & LIBSVM     & DC-SVM    & ML-SVM      & AML-SVM       \\ \hline
% 	Advertisement   & 0.67       & 0.90       & \bf{0.91}  & 0.90      & 231        & 610      & 213           & \bf{126}   \\
% 	Buzz            & 0.89       & 0.92       & \bf{0.95}  & \bf{0.95} & 26026      & 2524     & \bf{31 }      & 269        \\
% 	Clean (Musk)    & \bf{0.99}  & 0.94       & \bf{0.99}  & 0.93      & 82         & 95       & 94            & \bf{21}    \\
% 	Cod-RNA         & \bf{0.96}  & 0.93       & 0.94       & 0.95      & 1857       & 420      & \bf{13  }     & 75         \\
% 	Forest          & 0.92       & \bf{0.94}  & 0.88       & 0.88      & 353210     & 19970    & \bf{948}      & 2149       \\
% 	Letter          & 0.99       & \bf{1.00}  & 0.99       & 0.98      & 139        & 38       & 30            & \bf{14}    \\
% 	Ringnorm        & \bf{0.98}  & 0.95       & \bf{0.98}  & 0.97      & 26         & 38       & \bf{2 }       & 3          \\
% 	Twonorm         & \bf{0.98}  & 0.97       & \bf{0.98}  & 0.97      & 28         & 30       & \bf{1 }       & \bf{1}     \\ \hline
% \end{tabular}}
%   \end{center}
%   \caption{Performance measures and time for LIBSVM, DC-SVM, ML-SVM and AML-SVM on medium size benchmark data sets.}
% \end{table*}


